Inquisitive Action Logic

We introduce inquisitive action logic, InqAL, a multi-agent modal logic for reasoning about action. While traditional approaches focus on what properties of the outcome an agent can force, InqAL also captures what aspects of the outcome an agent determines through their actions. As we argue, such claims of agentive determination are naturally analyzed as modal claims involving questions. Technically, InqAL is a multi-agent extension of inquisitive neighborhood logic based on concurrent game structures. With respect to statements, it is expressively equivalent to the individual-agent fragment of the socially friendly coalition logic recently proposed by Goranko and Enqvist. We present an axiomatization of InqAL and prove completeness and decidability via the finite model property. Along the way, we establish a representation theorem for actual effectivity functions, associating to an agent the sets of outcomes corresponding to their possible actions; we give exact conditions under which a multi-agent neighborhood frame arises from a concurrent game structure.

==> eptcsdata.tex <==
\providecommand{\firstpage}{222}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.13}{10.4204/EPTCS.447.13}}

